On the Orr-Sommerfeld Equation with Linear Profile

The Orr-Sommerfeld equation with linear profile on the finite interval is considered. The behavior of the spectrum of this problem is completely investigated for large Reynolds numbers. The limit curves are found to which the eigenvalues concentrate and the counting eigenvalue functions along these curves are obtained.

==> pic_model/SPECTRUM.TEX <==
\put(0.000,-1.933){\circle*{0.03}}
\put(0.000,-1.852){\circle*{0.03}}
\put(0.000,-1.772){\circle*{0.03}}
\put(0.000,-1.694){\circle*{0.03}}
\put(0.000,-1.617){\circle*{0.03}}
\put(0.000,-1.542){\circle*{0.03}}
\put(0.000,-1.468){\circle*{0.03}}
\put(0.000,-1.395){\circle*{0.03}}
\put(0.000,-1.325){\circle*{0.03}}
\put(0.860,-0.081){\circle*{0.03}}
\put(0.000,-1.255){\circle*{0.03}}
\put(0.000,-1.187){\circle*{0.03}}
\put(0.755,-0.142){\circle*{0.03}}
\put(0.000,-1.121){\circle*{0.03}}
\put(0.669,-0.191){\circle*{0.03}}
\put(0.000,-1.056){\circle*{0.03}}
\put(0.592,-0.235){\circle*{0.03}}
\put(0.000,-0.993){\circle*{0.03}}
\put(0.523,-0.275){\circle*{0.03}}
\put(0.000,-0.930){\circle*{0.03}}
\put(0.458,-0.313){\circle*{0.03}}
\put(0.000,-0.870){\circle*{0.03}}
\put(0.397,-0.348){\circle*{0.03}}
\put(0.000,-0.810){\circle*{0.03}}
\put(0.339,-0.382){\circle*{0.03}}
\put(0.000,-0.752){\circle*{0.03}}
\put(0.283,-0.414){\circle*{0.03}}
\put(-0.001,-0.695){\circle*{0.03}}
\put(0.230,-0.445){\circle*{0.03}}
\put(0.178,-0.475){\circle*{0.03}}
\put(0.001,-0.640){\circle*{0.03}}
\put(0.128,-0.504){\circle*{0.03}}
\put(0.079,-0.532){\circle*{0.03}}
\put(0.029,-0.563){\circle*{0.03}}
\put(0.001,-0.585){\circle*{0.03}}
\put(-0.031,-0.559){\circle*{0.03}}
\put(-0.079,-0.532){\circle*{0.03}}
\put(-0.128,-0.504){\circle*{0.03}}
\put(-0.178,-0.475){\circle*{0.03}}
\put(-0.230,-0.445){\circle*{0.03}}
\put(-0.283,-0.414){\circle*{0.03}}
\put(-0.339,-0.382){\circle*{0.03}}
\put(-0.397,-0.348){\circle*{0.03}}
\put(-0.458,-0.313){\circle*{0.03}}
\put(-0.523,-0.275){\circle*{0.03}}
\put(-0.592,-0.235){\circle*{0.03}}
\put(-0.669,-0.191){\circle*{0.03}}
\put(-0.755,-0.142){\circle*{0.03}}
\put(-0.860,-0.081){\circle*{0.03}}


==> pic_orsom/SPECTRUM.TEX <==
\put(0.000,-1.934){\circle*{0.03}}
\put(0.000,-1.853){\circle*{0.03}}
\put(0.000,-1.772){\circle*{0.03}}
\put(0.000,-1.694){\circle*{0.03}}
\put(0.000,-1.617){\circle*{0.03}}
\put(0.000,-1.542){\circle*{0.03}}
\put(0.000,-1.468){\circle*{0.03}}
\put(0.000,-1.396){\circle*{0.03}}
\put(0.000,-1.325){\circle*{0.03}}
\put(0.000,-1.255){\circle*{0.03}}
\put(0.000,-1.187){\circle*{0.03}}
\put(0.774,-0.214){\circle*{0.03}}
\put(0.000,-1.121){\circle*{0.03}}
\put(0.711,-0.093){\circle*{0.03}}
\put(0.000,-1.056){\circle*{0.03}}
\put(0.608,-0.299){\circle*{0.03}}
\put(0.000,-0.993){\circle*{0.03}}
\put(0.000,-0.930){\circle*{0.03}}
\put(0.551,-0.190){\circle*{0.03}}
\put(0.471,-0.370){\circle*{0.03}}
\put(0.000,-0.870){\circle*{0.03}}
\put(0.350,-0.434){\circle*{0.03}}
\put(0.000,-0.811){\circle*{0.03}}
\put(0.417,-0.268){\circle*{0.03}}
\put(0.000,-0.752){\circle*{0.03}}
\put(0.239,-0.493){\circle*{0.03}}
\put(0.002,-0.695){\circle*{0.03}}
\put(0.297,-0.336){\circle*{0.03}}
\put(0.136,-0.548){\circle*{0.03}}
\put(-0.001,-0.639){\circle*{0.03}}
\put(0.040,-0.602){\circle*{0.03}}
\put(0.187,-0.394){\circle*{0.03}}
\put(-0.040,-0.601){\circle*{0.03}}
\put(0.000,-0.534){\circle*{0.03}}
\put(0.080,-0.443){\circle*{0.03}}
\put(0.000,-0.455){\circle*{0.03}}
\put(-0.136,-0.548){\circle*{0.03}}
\put(-0.080,-0.443){\circle*{0.03}}
\put(-0.239,-0.493){\circle*{0.03}}
\put(-0.187,-0.394){\circle*{0.03}}
\put(-0.350,-0.434){\circle*{0.03}}
\put(-0.298,-0.335){\circle*{0.03}}
\put(-0.471,-0.370){\circle*{0.03}}
\put(-0.417,-0.268){\circle*{0.03}}
\put(-0.608,-0.299){\circle*{0.03}}
\put(-0.774,-0.214){\circle*{0.03}}
\put(-0.551,-0.190){\circle*{0.03}}
\put(-0.711,-0.093){\circle*{0.03}}

